Beyond the Known: Novel Class Discovery for Open-world Graph Learning

Node classification on graphs is of great importance in many applications. Due to the limited labeling capability and evolution in real-world open scenarios, novel classes can emerge on unlabeled testing nodes. However, little attention has been paid to novel class discovery on graphs. Discovering novel classes is challenging as novel and known class nodes are correlated by edges, which makes their representations indistinguishable when applying message passing GNNs. Furthermore, the novel classes lack labeling information to guide the learning process. In this paper, we propose a novel method Open-world gRAph neuraL network (ORAL) to tackle these challenges. ORAL first detects correlations between classes through semi-supervised prototypical learning. Inter-class correlations are subsequently eliminated by the prototypical attention network, leading to distinctive representations for different classes. Furthermore, to fully explore multi-scale graph features for alleviating label deficiencies, ORAL generates pseudo-labels by aligning and ensembling label estimations from multiple stacked prototypical attention networks. Extensive experiments on several benchmark datasets show the effectiveness of our proposed method.

==> Tables/table_1.tex <==
\renewcommand\arraystretch{2}
\begin{table}[t]
\caption{Performance comparison of all methods.}\label{table main}
\setlength{\tabcolsep}{1.1mm}{}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{\textbf{Dataset}}& \multirow{2}{*}{\textbf{Method}} & \textbf{SSL} & \textbf{UL} & \multicolumn{6}{c|}{\textbf{Open-SSL}}\\
\cline{3-10}
&  & \textbf{GCN} & \textbf{VGAE} & \multicolumn{2}{c}{\textbf{GCD}} & \multicolumn{2}{|c|}{\textbf{OpenNCD}} & \multicolumn{2}{c|}{\textbf{\ours{}}}\\
\cline{2-10}
& Prior & No & Yes & Yes & No & Yes & No & Yes & No \\
\hline
\multirow{3}{*}{\textbf{Cora}} & All & 39.29 & 50.60 & 48.08 & 50.67 & 51.03 & 50.25 & \textbf{71.39} & \underline{69.91}\\
\cline{2-10}
& Known & 67.31 & 49.48 & 51.69 & 54.31 & 50.56 & 61.31 & \textbf{76.97} & \underline{73.60}\\
\cline{2-10}
& Novel  &  0.00 & 52.22 & 43.03 & 45.50 & 51.67 & 34.75 & \textbf{65.71} & \underline{64.72} \\
\cline{2-10}
\hline
\multirow{3}{*}{\textbf{BlogCatalog}} & All & 26.04 &38.18 & 37.91 & 37.79 & 42.73 & 42.83 & \textbf{73.76} & \underline{70.23}\\
\cline{2-10}
& Known & 70.28 & 25.03 & 27.13 & 26.00 & 34.84 & 34.55 & \textbf{88.46} & \underline{87.39} \\
\cline{2-10}
& Novel & 0.00 & 45.92 & 44.25 & 44.73 & 47.37 & 47.70 & \textbf{65.11} & \underline{60.14}\\
\hline
% \multirow{3}{*}{\textbf{\thead{Amazon \\ Computer}}} & All & 52.98 & 55.54 & 53.97 & 54.13 & 66.96 & 77.92& \underline{81.61} & \textbf{81.78}\\
% \cline{2-10}
% & Known & 81.30 & 37.94 & 47.71 & 47.44 & 67.35 & 81.86  & \textbf{88.03} & 85.91 \\
% \cline{2-10}
% & Novel & 0.00 & \textbf{88.48} & 66.23 & 66.65 & 66.23 & 70.54 & 69.60 & \underline{74.07} \\
% \hline
\multirow{3}{*}{\textbf{\thead{Amazon \\ Photo}}} & All & 56.69 & 66.35 & 70.52 & 70.66 & 67.41 & 66.55 & \textbf{88.05} & \underline{84.09}\\
\cline{2-10}
& Known & 93.44 & 65.89 & 71.98 & 71.98 & 66.75 & 74.67 & \textbf{95.36} & \underline{92.71} \\
\cline{2-10}
& Novel & 0.00 & 67.06 & 68.27 & 68.44 & 68.43 & 54.04 & \textbf{76.77} & \underline{70.79} \\
\cline{2-10}

% \hline
% \multicolumn{2}{|c|}{Average performance} & 39.22 & 51.19 & 51.42 & 52.23 & 51.10 & 51.38 & \textbf{77.95} & \underline{74.84} \\
\hline
\multicolumn{2}{|c|}{Average Novel} & 0.00 & 55.06 & 51.85 & 52.89 & 55.30 & 45.95 & \textbf{69.20} & \underline{65.21}\\
\hline

\end{tabular}
\end{table}


==> method_copy.tex <==
\section{Problem Formulation}
\textbf{Notations.} A graph is represented as $G=(\mathcal{V},\mathcal{E},\mathbf{X})$, where $\mathcal{V}=\{v_i\}_{i=1,...,N}$ is a node set representing nodes in a graph, $e_{i,j}=(v_i,v_j) \in \mathcal{E}$ is an edge indicating the relationship between two nodes and $\mathbf{x}_i \in \mathbf{X}$ indicates content features associated with each node $v_i$. 
% The topological structure of a graph $G$ can be represented by an adjacency matrix $A$, where $A_{i,j}=1$ if $(v_i,v_j) \in E$, otherwise $A_{i,j}=0$.

\subsubsection{\ourtopic{}.} The node set $\mathcal{V}$ is composed of labeled training nodes $\mathcal{V}_{L}$ and unlabeled test nodes $\mathcal{V}_{U}$, which belong to class set $\mathcal{Y}^L$ and $\mathcal{Y}^U$ respectively. In open-world scenarios, novel class can emerge on the unlabeled nodes, i.e. $\mathcal{Y}^L \subset \mathcal{Y}^U$. The aim of \ourtopic{} is to discover novel classes automatically and classify the unlabeled nodes into known classes ($\mathcal{Y}^L$) or novel classes ($\mathcal{Y}^U-\mathcal{Y}^L$).


\section{Methodology}

\noindent \textbf{Overview.} The framework of our proposed method \ours{} is shown in Figure \ref{Figure model}. \revise{\ours{} first employs the prototypical attention network (PAN) to eliminate correlations between novel and known classes by blocking message passing. Given representative nodes (prototypes) extracted by prototype learning, PAN performs semi-supervised clustering on the prototype graph of relatively small size, efficiently obtaining group assignments of prototypes and nodes. Message passing between groups are blocked by the group attention mechanism to generate separable representations.} \revise{\ours{} further eases the lack of labeling information by the pseudo-label generator, which aligns and ensembles multiple clustering results. Pseudo-labeling guides the open-world learning through structure refining. To improve robustness against pseudo-labeling noise, we further enforce the prediction consistency regardless of permutation over the structure information.}



\subsection{Prototypical Attention Network}
\revise{The prototypical attention network clusters nodes into groups and eliminates correlations between  classes by blocking message passing between groups. Since the number of novel classes is unknown, we have to repeatedly perform clustering on graphs to search for the optimal cluster granularity by fitting the labeling information, which can be time-consuming. To ease the computation burden, we extract representative nodes through prototype learning and conduct semi-supervised clustering on the small prototype graph instead of the large whole graph. The cluster result of nodes are approximated from that of prototypes, which are employed to block message passing according to the group attention mechanism.}

% mines pairwise is unknown,similarity metric from known classes, facilitating detecting heterophily edges concerning novel classes. To alleviate the computational burden of optimizing similarity metric over all node pair repeatedly during the learning process, we first extract prototypes (representative nodes) on graphs. The optimization of similarity metric is conducted on representative prototypes instead of the whole node set. The heterophily scores of edges are calculated by the optimized similarity metric, which serve as attention weights to guide message passing.

\subsubsection{Prototype Learning.} Given a node with feature $\mathbf{x}_i$ and a set of trainable prototypes $\mathcal{C} = \{\mathbf{c}_1, \mathbf{c}_2, \cdots \mathbf{c}_{N_{proto}} \}$, we compute the representativeness of the prototype to node as follows,
\begin{equation}
    \mathbf{p}_{ij} = \frac{\exp({\mathbf{x}_i^T \mathbf{c}_j})}{\sum_{k=1}^{N_{proto}}{\exp({\mathbf{x}_i^T \mathbf{c}_k}})}.
    \label{Eq n2p}
\end{equation}
To ensure each prototype is representative of a set of nodes on graphs, we regularize the marginal distribution of prototype assignments to be close to a balanced prior by Kullback-Leibler (KL) divergence,
\begin{equation}
    \mathcal{L}_{reg}=KL[(\frac{1}{N_{proto}} \cdot \mathbf{1}) || (\frac{1}{|\mathcal{V}|}\sum_{i=1}^{|\mathcal{V}|}\mathbf{p}_i)],
    \label{loss reg}
\end{equation}
% \begin{equation}
%     \begin{aligned}
%         \mathcal{L}_{reg}=KL(\mathbf{p}_{proto} || \mathbf{p}_{prior}) \\
%         \mathbf{p}_{prior}=\frac{1}{N_{proto}}\mathbf{1} \\
%         \mathbf{p}_{proto}=\frac{1}{|\mathcal{V}|}\sum_{i=1}^{|\mathcal{V}|}\mathbf{p}_i
%     \end{aligned}
% \end{equation}
where $\mathbf{1} \in R^{N_{proto}}$ represents the all-ones vector.
% We further conduct contrastive learning to ensure only intrinisically important features on graphs are captured by prototypes. The probability representing the importance of each feature dimension is calculated according to its appearance frequency on influential nodes,
% \begin{equation}
%     \begin{aligned}
%         p^f_j = &\frac{s^f_{max}-s^f_{j}}{s^f_{max}-s^f_{min}}, \\ 
%         s^f_j=\log & \sum_{i\in \mathcal{V}} |\mathbf{x}_{ij}| \cdot \deg(i),
%     \end{aligned}
% \end{equation}
% where $\deg(i)$ is the degree of node $i$. $s^f_{max}$ and $s^f_{min}$ is the maximum and minimum value of $s^f_i$ respectively. We perform feature-level augmentation according to the importance probability and conduct contrastive learning between different views,
% \begin{equation}
%         \mathcal{L}_{fcon} = \sum_{i=1}^{|\mathcal{V}|}KL(\mathbf{p}_{i} || \hat{\mathbf{p}}_{i}),
%         \label{loss con}
% \end{equation}
% where $\hat{\mathbf{p}}_{i}$ is the assignment probability of the augmented feature vector. 
The relationships between prototypes are calculated according to their associated nodes. Each node is regarded as an associated instance of prototypes with the top k largest representativeness score. The associated nodes of each prototype is represented as,
\begin{equation}
    \Gamma(\mathbf{c}_i) = \{v_i | \mathbf{c}_i\in TOP_{K}(v_i)\}
\end{equation}
The relationship of two prototypes can be calculated from the similarity between their associated nodes:
\begin{equation}
    S_{ij} = \frac{|\Gamma(\mathbf{c}_i) \cap \Gamma(\mathbf{c}_j)|}{|\Gamma(\mathbf{c}_i) \cup \Gamma(\mathbf{c}_j)|}.
\end{equation}

\subsubsection{Semi-supervised Prototypical Clustering.} \revise{Known classes provide the labeling granularity, too fine-grained (coarse-grained) clustering can lead to poor accuracy on labeled nodes. We search for the optimal clustering granularity on the prototype graph $\{\mathcal{C},S\}$ by fitting the label information. Specifically, performing the clustering algorithm with granularity $\alpha_{cluster}$ can obtain,
\begin{equation}
    f_{cluster}(\alpha_{cluster}):\{\mathcal{C}, S\} \rightarrow{} \mathcal{C}^g,
\end{equation}
where $\mathcal{C}^g=\{\mathcal{C}_1^g,\cdots,\mathcal{C}_{N_{cluster}}^g\}$ is the set of prototype groups. For example, we can choose the spectral clustering with the number of clusters as the granularity parameter. Considering the $O(N^3)$ time complexity of spectral clustering, clustering on the small prototype graph instead of the large whole graph can ease computational burden significantly. The assignment probability of a node $v_i$ to a group $\mathcal{C}_k^g$ can be approximated as,
\begin{equation}
    \mathbf{p}^g_{ik} = \frac{\sum_{\mathbf{c}_j \in \mathcal{C}^g_k} \exp(\mathbf{x}_i^T\mathbf{c}_j)}{\sum_{\mathbf{c}_j \in \mathcal{C}} \exp(\mathbf{x}_i^T\mathbf{c}_j)}.
    \label{Eq groupassign}
\end{equation}
We match the prototype groups to known classes by the Hungarian algorithm \cite{Kuhn1955TheHM}, obtaining $f_{match}:\mathcal{C}^g \rightarrow{} \mathcal{Y}^L$. Then we search for the optimal clustering parameter that can achieves the highest accuracy over labeled nodes,
\begin{equation}
\begin{aligned}
\alpha_{cluster}* = &\mathop{\arg\min}\limits_{\alpha_{cluster}} \sum_{v_i\in \mathcal{V}_L} Acc(\hat{y}_i,y_i), \\
    \hat{y}_i=&f_{match}(\mathop{\arg\max}\limits_{k}\mathbf{p}^g_{ik})
\end{aligned}
\end{equation}
where $\hat{y}_i$ is the prediction made according to the group assignment. Groups do not match any known class are regarded as discovered novel classes.}


% , we take graph clustering methods as a similarity metric to evaluate whether any two prototypes coming from the same class. Prototypes do not share the same class with any known class prototype belong to novel classes. 

% The known class information associated with prototypes provides supervision for searching the optimal similarity metric by controlling the clustering parameters. Specifically, the graph clustering method detect groups over the prototype graph,
% \begin{equation}
%     f_{cluster}(\alpha_{cluster}):\{\mathcal{C}, S\} \rightarrow{} \mathcal{C}^g,
% \end{equation}
% where $\mathcal{C}^g=\{\mathcal{C}_1^g,\cdots,\mathcal{C}_{N_{cluster}}^g\}$ is the set of prototype groups. $f_{cluster}(\alpha_{cluster})$ is the clustering algorithm with hyperparameter $\alpha_{cluster}$. For example, we can choose the Louvain algorithm \cite{Blondel2008FastUO}  with the clustering resolution as the controllable parameter. Each detected group is regarded as the set of similar prototypes coming from the same class. To ensure the clustering algorithm learns the proper intra-class (inter-class) similarities, we search for the optimal hyperparametr such that nodes coming from the same known class (different known classes) are assigned to the same prototype group (different groups). The assignment probability from a node $v_i$ to a prototype group $\mathcal{C}_k^g$ can be calculated as,
% \begin{equation}
%     \mathbf{p}^g_{ik} = \frac{\sum_{\mathbf{c}_j \in \mathcal{C}^g_k} \exp(\mathbf{x}_i^T\mathbf{c}_j)}{\sum_{\mathbf{c}_j \in \mathcal{C}} \exp(\mathbf{x}_i^T\mathbf{c}_j)}.
%     \label{Eq groupassign}
% \end{equation}
% We match the prototype groups to known classes by the Hungarian algorithm \cite{Kuhn1955TheHM}, obtaining $f_{match}:\mathcal{C}^g \rightarrow{} \mathcal{Y}^L$. Then we search for the optimal clustering parameter that can achieves the highest accuracy over labeled nodes,
% \begin{equation}
% \begin{aligned}
% \alpha_{cluster}* = &\mathop{\arg\min}\limits_{\alpha_{cluster}} \sum_{v_i\in \mathcal{V}_L} Acc(\hat{y}_i,y_i), \\
%     \hat{y}_i=&f_{match}(\mathop{\arg\max}\limits_{k}\mathbf{p}^g_{ik})
% \end{aligned}
% \end{equation}
% where $\hat{y}_i$ is the prediction made according to the group assignment. Prototype groups do not match any known class are regarded as discovered novel classes.

\subsubsection{Group Attention Mechanism.} \revise{To learn compact representations, we propose the group attention mechanism to guide message passing. The group attention mechanism calculates the attention score according to the group assignment similarities,
\begin{equation}
    \begin{aligned}
        \alpha_{ij} = \mathrm{softmax} & (e_{ij})=\frac{\exp{(e_{ij})}}{\sum_{k\in N(i)} \exp{(e_{ik})}}, \\
        e_{ik} =& \cos{(\mathbf{p}_i^g, \mathbf{p}_k^g)}.
    \end{aligned}
\end{equation}
Since group assignments are approximations of ground-truth label information, the group assignment similarity between novel and known class nodes are relatively low. Consequently, aggregating information according to the group assignments can eliminate correlations classes and obtain compact representations,
\begin{equation}
    \mathbf{h}_i = \sum_{j\in N(i)} \alpha_{ij} \mathbf{W}\mathbf{x}_j.
    \label{Eq groupatt}
\end{equation}
To acquire high-order neighbor information, we stack multiple layers of the prototypical attention network which are trained by the cross-entropy loss,
\begin{equation}
    \mathcal{L}_{ce} = \sum_{v_i\in\mathcal{V}}\sum_{l=1}^L-\log \mathbf{p}^{g(l)}_{iy_i}
    \label{loss ce}
\end{equation}
Consequently, we have access to a list of prediction results as well as node embeddings, $\{(\mathbf{p}^{g(1)},\mathbf{h}^{(1)}),...,(\mathbf{p}^{g(L)},\mathbf{h}^{(L)})\}$, calculated at different scales.}
% . We train the group attention network with the cross-entropy loss,
% \begin{equation}
%     \mathcal{L}_{ce} = \sum_{v_i\in\mathcal{V}}\sum_{l=1}^L-\log \mathbf{p}^{g(l)}_{iy_i}
%     \label{loss ce}
% \end{equation}}
% block message passing between classes and 
% Besides attribute features, high-order neighbor information \cite{Kipf2016SemiSupervisedCW,Chen2020ConvolutionalKN} are also important for node classification as well as novel class discovery. However, naively aggregating the neighbor information with existing graph convolution layers \cite{kipf2016semi,huang2018adaptive,Izadi2020OptimizationOG,luan2021heterophily,biology,Bruna2013SpectralNA,Niepert2016LearningCN} are not guaranteed to contain knowledge about how to discover novel classes. 

% Message passing operator of the graph convolution layer tends to make node embeddings similar. To distinguish novel class nodes from others, we summarize two properties the graph convolution layer should possess: (1) Allow messages to pass within nodes from the same novel class. (2) Block information flow between nodes belonging to a novel class and those from both known classes and other novel classes. Therefore, we propose the following attention mechanism,
% \begin{equation}
%     \begin{aligned}
%         \alpha_{ij} = \mathrm{softmax} & (e_{ij})=\frac{\exp{(e_{ij})}}{\sum_{k\in N(i)} \exp{(e_{ik})}}, \\
%         e_{ik} =& \cos{(\mathbf{p}_i^g, \mathbf{p}_k^g)},
%     \end{aligned}
% \end{equation}
% where we utilize the cosine similarity of prototype group assignment probabilities as the attention weights. Given the clustering algorithm evaluating intra-class (inter-class) similarities learned from known classes, nodes representing novel classes are assigned to distinct prototype groups compared to nodes from other classes, based on the evaluation of their similarities. Consequently, the attention weights between novel class nodes and nodes from other classes are low. The similar applies for the high attention scores between nodes from the same novel classes. Then we aggregate neighborhood information according to the attention weights,
% \begin{equation}
%     \mathbf{h}_i = \sum_{j\in N(i)} \alpha_{ij} \mathbf{W}\mathbf{x}_j.
%     \label{Eq groupatt}
% \end{equation}

% To acquire high-order neighbor information, we stack multiple layers of the prototypical Attention Network. Consequently, we have access to a list of prediction results as well as node embeddings, $\{(\mathbf{p}^{g(1)},\mathbf{h}^{(1)}),...,(\mathbf{p}^{g(L)},\mathbf{h}^{(L)})\}$. We train the group attention network with the cross-entropy loss,
% \begin{equation}
%     \mathcal{L}_{ce} = \sum_{v_i\in\mathcal{V}}\sum_{l=1}^L-\log \mathbf{p}^{g(l)}_{iy_i}
%     \label{loss ce}
% \end{equation}
% since novel class nodes are assigned to different prototype groups. To transfer the intra-class (inter-class) similarity relationships mined from the known classes for novel category discovery

\subsection{Pseudo-label guided Open-world Learning}
\revise{To mitigate the lack of novel class labeling information, we generate reliable pseudo-labels to guide the open-world graph learning. The generation process of pseudo-labels is shown in the pseudo-label generator part, while the utilization of pseudo-labels is detailed in the data-centric learning part.}


\subsubsection{Pseudo-label Generator.} \revise{To
bring into full play the rich information captured at different scales, \ours{} ensembles prediction results estimated by multiple stacked prototypical attention networks. However, ensembling multiple group assignment results is non-trivial. Due to the unsupervised nature of novel class discovery, groups from different layers are not aligned, even the number of groups varies from layer to layer.}

\revise{We overcome these challenges through the proposed padding, aligning and suppressing operation. Given the set of predictions $\{\mathbf{p}^{g(1)},...,\mathbf{p}^{g(L)} \}$, we first pad them with zero vectors such that they have the same number of prototype groups. Then we align and ensemble predictions from different layers by the Hungarian algorithm,
\begin{equation}
    \hat{\mathbf{p}}_{i,j}^{esm} = \frac{1}{L}\sum_{k=1}^L{\mathbf{p}^{g(k)}_{i,f_{match(1,k)}(j)}},
\end{equation}
where $f_{match(1,k)}(j)$ denotes the prototype group ID in the k-th layer that corresponds to the j-th group in the initial layer. Groups which only exist in a certain layer or associates with almost no nodes can be regarded as detection noise, we suppress neurons respond to these noisy groups,
\begin{equation}
    \begin{aligned}
        \mathbf{p}^{esm}_i =& \hat{\mathbf{p}}^{esm}_{i,\mathbf{M}}\\
        \mathbf{M} = \{j | \frac{1}{|\mathcal{V}|}&\sum_{v_i\in \mathcal{V}}\hat{\mathbf{p}}_{ij}^{esm}>\eta\}
    \label{Eq ensemble}
    \end{aligned}
\end{equation}
where $\eta$ is the hyperparameter. After obtaining the pseudo-labels for all nodes by ensemble inference, we select the top $\gamma$ percentage of nodes with the highest prediction probability in each class, resulting in a subset of nodes called the top confident node subset $\eta^k$,
\begin{equation}
    \begin{aligned}
        \Lambda^k = \{v_i|v_i \in \hat{\Lambda}^k,& Rank|_{\hat{\Lambda}^k} (\mathbf{p}_{ik}^{esm}) \leq \gamma*|\hat{\Lambda}^k|\} \\
        \hat{\Lambda}^k = &\{v_i| \mathop{\arg\max}\limits_{j} \mathbf{p}_{ij}^{esm}=k\} \\
    \end{aligned}
\end{equation}
where $Rank|_{\hat{\Lambda}^k} (\mathbf{p}_{ik}^{esm})$ represents the ranking of prediction confidence of node $v_i$ within the k-th group $\hat{\Lambda}^k$.
}

\begin{algorithm} 
\LinesNumbered
\caption{\ours{}}
\label{Pseudocode}
\KwData{Graph $G=(\mathcal{V},\mathcal{E},\mathbf{X})$, Labeled training nodes $ (\mathcal{V}_L,\mathcal{Y}^L)$} 
\KwResult{Predictions of unlabeled nodes $(\mathcal{V}_U,\hat{\mathcal{Y}}^U)$ where new labels can emerge, i.e. $\mathcal{Y}^L \subset \hat{\mathcal{Y}}^U$}
\BlankLine
Randomly initialize model parameters\;
\Repeat{Convergence or iteration number reaches the threshold}{
    \For{$l=1$ to $L$}{
            Calculate group assignments $\mathbf{p}^{g(l)}$ according to Eq. (\ref{Eq groupassign})\;
            Calculate node embeddings $\mathbf{h}^{(l)}$ according to Eq. (\ref{Eq groupatt}) \;}
    % Calculate loss  $\mathcal{L}$ according to Eq. $\ref{Eq loss}$\;
    Update model parameters according to loss defined in Eq. ($\ref{Eq loss}$)\;
    Update the graph structure according to Eq. (\ref{Eq structure})\;
}
Predict test node labels by ensemble inference in Eq. (\ref{Eq ensemble})\;
\end{algorithm}

 
\revise{\subsubsection{Data-centric Open-world Learning.} We guide open-world learning from the data-centric perspective by refining graph structures according to pseudo-labels, such that pseudo-label information can be propagated to other nodes during message passing on graphs. Specifically, we recover intra-class (eliminate inter-class) edges to increase intra-class (decrease inter-class) similarities according to pseudo-labeling, which facilitates distinguishing novel classes from others. }

\revise{Considering that recovering too many edges can lead to over-smoothing, we only select the top $\mu$ percent of intra-class node pair with the lowest similarities as recovered edges,
\begin{equation}
    \begin{aligned}
        \mathcal{E}^k_{rc} = \{(\Lambda_i^k,\Lambda_j^k)&|Rank(S^k_{ij}) \leq \mu*|\Lambda^k|^2\}, \\
        S^k_{ij} = \frac{1}{L}\sum_{l=1}^L &\cos{(\mathbf{p}^{(l)}_{\Lambda_i^k}, \mathbf{p}^{(l)}_{\Lambda_j^k})},\\
        \mathcal{E}_{rc} &= \cup_k \mathcal{E}^k_{rc},
    \end{aligned}
\end{equation}
where the similarity between nodes $S^k_{ij}$ is calculated according to their relationships to prototypes calculated in Equation \ref{Eq n2p}. Consequently, edges between intra-class nodes associated to different prototypes are recovered, which increases similarities between prototypes related to the same class and facilitates better semi-supervised prototypical clustering. We further eliminates inter-class edges between top confident nodes,
\begin{equation}
    \mathcal{E}_{rm} = \{(\Lambda_i^{k_1},\Lambda_j^{k_2})|(\Lambda_i^{k_1},\Lambda_j^{k_2})\in\mathcal{E},k_1 \neq k_2\}.
\end{equation}
The refined structure can be formulated as,
\begin{equation}
    \mathcal{E}^{upd} = \mathcal{E} - \mathcal{E}_{rm} + \mathcal{E}_{rc}.
    \label{Eq structure}
\end{equation}
To make \ours{} robust to the noise introduced during the structure refining process, we introduce the permutation-consistent training loss, which augments the structure information with the adaptive  augmentation technique \cite{Zhu2020GraphCL} and regularizes the prediction consistency between different views,
\begin{equation}
    \mathcal{L}_{con} = \sum_{v_i \in \mathcal{V}}\sum_{l=1}^L KL(\mathbf{p}_i || \bar{\mathbf{p}}_i)+KL(\mathbf{p}^{g(l)}_i || {\bar{\mathbf{p}}^{g(l)}_i}),
    \label{loss scon}
\end{equation}
where $\mathbf{p}_i$ and $\mathbf{p}_i^{aug}$ are the prototype assignment in the input graph and augmented graph. The overall training loss can be calulated as,
\begin{equation}
\mathcal{L}=\mathcal{L}_{ce}+\mathcal{L}_{reg}+\mathcal{L}_{con}
    \label{Eq loss}
\end{equation}
The final predictions on unlabeled nodes can be obtained based on Eq. (\ref{Eq ensemble}). The training process is summarized in Algorithm \ref{Pseudocode}.}



% \revise{As nodes from the same class but assigned to different prototypes are relatively less similar, recovering intra-class edges between nodes with different prototype assignments can enhance intra-class similarities. We calculate the prototype assignment probability similarity within the top confident node subset of each class,
% \begin{equation}
%     S^k_{ij} = \frac{1}{L}\sum_{l=1}^L \cos{(\mathbf{p}^{(l)}_{\Lambda_i^k}, \mathbf{p}^{(l)}_{\Lambda_j^k})},
% \end{equation}
% where $\mathbf{p}^{(l)}_{\Lambda_j}$ is the prototype assignment of node $\Lambda_j$ in the $l$-th layer. Then we select the top $\mu$ percent of node pair with the lowest assignment similarities as recovered edges,
% \begin{equation}
%     \begin{aligned}
%         \mathcal{E}^k_{rc} = \{(\Lambda_i^k,\Lambda_j^k)&|Rank(S^k_{ij}) \leq \mu*|\Lambda^k|^2\} \\
%         \mathcal{E}_{rc} &= \cup_k \mathcal{E}^k_{rc}
%     \end{aligned}
% \end{equation}
% We further eliminates heterophily edges between top confident nodes,
% \begin{equation}
%     \mathcal{E}_{rm} = \{(\Lambda_i^{k_1},\Lambda_j^{k_2})|(\Lambda_i^{k_1},\Lambda_j^{k_2})\in\mathcal{E},k_1 \neq k_2\}.
% \end{equation}
% The updated structure can be formulated as,
% \begin{equation}
%     \mathcal{E}^{upd} = \mathcal{E} - \mathcal{E}_{rm} + \mathcal{E}_{rc}.
%     \label{Eq structure}
% \end{equation}
% The updated structure is taken as input for finetuning and inference. To make \ours{} robust to the noise introduced during the structure updating process, we augment the updated structure with the adaptive  augmentation technique \cite{Zhu2020GraphCL} and regularizes the prediction consistency between different views of the updated structure information,
% \begin{equation}
%     \mathcal{L}_{scon} = \sum_{v_i \in \mathcal{V}}\sum_{l=1}^L KL(\mathbf{p}_i || \bar{\mathbf{p}}_i)+KL(\mathbf{p}^{g(l)}_i || {\bar{\mathbf{p}}^{g(l)}_i}),
%     \label{loss scon}
% \end{equation}
% where $\mathbf{p}_i$ and $\mathbf{p}_i^{aug}$ are the prototype assignment in the input graph and augmented graph. The overall training loss can be calulated as,
% \begin{equation}
% \mathcal{L}=\mathcal{L}_{ce}+\mathcal{L}_{reg}+\mathcal{L}_{fcon}+\mathcal{L}_{scon}
%     \label{Eq loss}
% \end{equation}
% The final predictions on unlabeled nodes can be obtained based on Eq. (\ref{Eq ensemble}). The training process is summarized in Algorithm \ref{Pseudocode}.}



% To facilitate more accurate novel class discovery and node classification, the homophily-enhanced structural ensemble learning further increases (decreases) intra-class (inter-class) similarities by refining the input graph structure based on prediction results. Considering the noisy nature of each layer's prediction results, we first align and ensemble the predictions from various layers. Subsequently, we selectively choose ensemble predictions that exhibit high confidence for the purpose of structure refinement.  

% \subsubsection{Ensemble Predictor with Alignment.}  Ensembles of different prototypical attention layers' predictions can boost the generalization performance and robustness since the classification of different classes might rely on different hops of neighborhood information. However, it is non-trivial as different prototypical attention network layer might map the same class to different prototype group IDs and different layers may have different numbers of prototype groups. To overcome this challenge, we first align different layers' prediction results through the Hungarian algorithm prior to the ensemble process. Given the set of predictions $\{\mathbf{p}^{g(1)},...,\mathbf{p}^{g(L)} \}$, we first pad them with zero vectors such that they have the same number of prototype groups. Then we calculate the ensemble inference results as follows,
% \begin{equation}
%     \hat{\mathbf{p}}_{:j}^{esm} = \frac{1}{L}\sum_{k=1}^L{\mathbf{p}^{g(k)}_{:f_{match(1,k)}(j)}},
% \end{equation}
% where $f_{match(1,k)}(j)$ denotes the prototype group ID in the k-th layer that corresponds to the j-th group in the initial layer. $\hat{\mathbf{p}}_{:j}^{esm}$ represents the j-th column of the prediction results. Prototype groups only exist in a certain layer are associated to a few or nearly zero nodes, which can be regarded as noisy prototype groups. We suppress neurons respond to these noisy prototypes,
% \begin{equation}
%     \begin{aligned}
%         \mathbf{p}^{esm}_i =& \hat{\mathbf{p}}^{esm}_{i,\mathbf{M}}\\
%         \mathbf{M} = \{j | \frac{1}{|\mathcal{V}|}&\sum_{v_i\in \mathcal{V}}\hat{\mathbf{p}}_{ij}^{esm}>\eta\}
%     \label{Eq ensemble}
%     \end{aligned}
% \end{equation}
% where $\eta$ is the hyperparameter. After obtaining the pseudo-labels for all nodes by ensemble inference, we select the top $\gamma$ percentage of nodes with the highest prediction assignment probability in each class, resulting in a subset of nodes called  the top confident node subset $\eta^k$,
% \begin{equation}
%     \begin{aligned}
%         \Lambda^k = \{v_i|v_i \in \hat{\Lambda}^k,& Rank|_{\hat{\Lambda}^k} (\mathbf{p}_{ik}^{esm}) \leq \gamma*|\hat{\Lambda}^k|\} \\
%         \hat{\Lambda}^k = &\{v_i| \mathop{\arg\max}\limits_{j} \mathbf{p}_{ij}^{esm}=k\} \\
%     \end{aligned}
% \end{equation}
% where $Rank|_{\hat{\Lambda}^k} (\mathbf{p}_{ik}^{esm})$ represents the ranking of assignment probability of node $v_i$ within the k-th prototype group $\hat{\Lambda}^k$.

% \subsubsection{Structure Refinement via Pseudo-labeling.} Based on the top confident node subset produced by ensemble inference, the structural learning module recovers missing homophily edges to enhance   intra-class similarities while eliminating noisy heterophily edges to diminish inter-class similarities. This process facilitates better separating each class from others.

% As nodes from the same class but assigned to different prototypes are relatively less similar, recovering intra-class edges between nodes with different prototype assignments can enhance intra-class similarities. We calculate the prototype assignment probability similarity within the top confident node subset of each class,
% \begin{equation}
%     S^k_{ij} = \frac{1}{L}\sum_{l=1}^L \cos{(\mathbf{p}^{(l)}_{\Lambda_i^k}, \mathbf{p}^{(l)}_{\Lambda_j^k})},
% \end{equation}
% where $\mathbf{p}^{(l)}_{\Lambda_j}$ is the prototype assignment of node $\Lambda_j$ in the $l$-th layer. Then we select the top $\mu$ percent of node pair with the lowest assignment similarities as recovered edges,
% \begin{equation}
%     \begin{aligned}
%         \mathcal{E}^k_{rc} = \{(\Lambda_i^k,\Lambda_j^k)&|Rank(S^k_{ij}) \leq \mu*|\Lambda^k|^2\} \\
%         \mathcal{E}_{rc} &= \cup_k \mathcal{E}^k_{rc}
%     \end{aligned}
% \end{equation}
% We further eliminates heterophily edges between top confident nodes,
% \begin{equation}
%     \mathcal{E}_{rm} = \{(\Lambda_i^{k_1},\Lambda_j^{k_2})|(\Lambda_i^{k_1},\Lambda_j^{k_2})\in\mathcal{E},k_1 \neq k_2\}.
% \end{equation}
% The updated structure can be formulated as,
% \begin{equation}
%     \mathcal{E}^{upd} = \mathcal{E} - \mathcal{E}_{rm} + \mathcal{E}_{rc}.
%     \label{Eq structure}
% \end{equation}
% The updated structure is taken as input for finetuning and inference. To make \ours{} robust to the noise introduced during the structure updating process, we augment the updated structure with the adaptive  augmentation technique \cite{Zhu2020GraphCL} and regularizes the prediction consistency between different views of the updated structure information,
% \begin{equation}
%     \mathcal{L}_{scon} = \sum_{v_i \in \mathcal{V}}\sum_{l=1}^L KL(\mathbf{p}_i || \bar{\mathbf{p}}_i)+KL(\mathbf{p}^{g(l)}_i || {\bar{\mathbf{p}}^{g(l)}_i}),
%     \label{loss scon}
% \end{equation}
% where $\mathbf{p}_i$ and $\mathbf{p}_i^{aug}$ are the prototype assignment in the input graph and augmented graph. The overall training loss can be calulated as,
% \begin{equation}
% \mathcal{L}=\mathcal{L}_{ce}+\mathcal{L}_{reg}+\mathcal{L}_{fcon}+\mathcal{L}_{scon}
%     \label{Eq loss}
% \end{equation}
% The final predictions on unlabeled nodes can be obtained based on Eq. (\ref{Eq ensemble}). The training process is summarized in Algorithm \ref{Pseudocode}.

% \begin{algorithm} 
% \LinesNumbered
% \caption{\ours{}}
% \label{Pseudocode}
% \KwData{Graph $G=(\mathcal{V},\mathcal{E},\mathbf{X})$, Labeled training nodes $ (\mathcal{V}_L,\mathcal{Y}^L)$} 
% \KwResult{Predictions of unlabeled nodes $(\mathcal{V}_U,\hat{\mathcal{Y}}^U)$ where new labels can emerge, i.e. $set(\mathcal{Y}^L) \subset set(\hat{\mathcal{Y}}^U)$}
% \BlankLine
% Randomly initialize model parameters\;
% \Repeat{Convergence or iteration number reaches the threshold}{
%     \For{$l=1$ to $L$}{
%             Calculate group assignments $\mathbf{p}^{g(l)}$ according to Eq. (\ref{Eq groupassign})\;
%             Calculate node embeddings $\mathbf{h}^(l)$ according to Eq. (\ref{Eq groupatt}) \;}
%     % Calculate loss  $\mathcal{L}$ according to Eq. $\ref{Eq loss}$\;
%     Update model parameters according to loss defined in Eq. ($\ref{Eq loss}$)\;
%     Update the graph structure according to Eq. (\ref{Eq structure})\;
% }
% Predict test node labels by ensemble inference in Eq. (\ref{Eq ensemble})\;
% \end{algorithm}



% % Unlike closed-world settings, ensemble can be simply achieved by mean averaging the prediction results from different modules. Different layer of PAN may map the same class to different prototype group ID. To overcome this challenge, we first align different layer's prediction through the Hungarian algorithm before mean averaging ensembling. Given the layer-wise predictions, we align other layer's prediction results to the first layer,
% % We search for the clustering parameter that can achieve the highest accuracy over known class nodes, 
% % We first utilize Hungarian algorithm \cite{Kuhn1955TheHM} to match the known classes with the prototype groups, 


% % and search for the clustering parameter that can achieve the highest accuracy over known class nodes, 


% % the prototype groups not matched with any known class is regarded as novel classes.

% % nodes coming from the same known class should be assigned to the same prototype group, while those belonging to different classes should be assigned to different groups. The assignment probability from a node $v_i$ to a prototype group $\mathcal{C}_k^g$ can be calculated as,
% % \begin{equation}
% %     \mathbf{p}^g_{ik} = \frac{\sum_{\mathbf{c}_j \in \mathcal{C}^g_k} \exp(\mathbf{x}_i^T\mathbf{c}_j)}{\sum_{\mathbf{c}_j \in \mathcal{C}} \exp(\mathbf{x}_i^T\mathbf{c}_j)}.
% % \end{equation}
% % We utilize the Hungarian algorithm \cite{Kuhn1955TheHM} to match the known classes with the prototype groups, the prototype groups not matched with any known class is regarded as novel classes. We search for the clustering parameter that can achieves the highest accuracy over known class nodes,
% % \begin{equation}
% %     \alpha_{cluster} = \mathop{\arg\min}\limits_{\alpha_{cluster}} \sum_{v_i\in \mathcal{V}_L} CE(\mathbf{p}^g_{i},y_i),
% % \end{equation}
% % where $CE$ represents the cross-entropy loss.



% % is calculated to form an affinity matrix. Some graph based clustering methods can then be utilized to detect the
% % densely connected prototypes, which are regarded as prototype groups. A simple way is to find the prototype groups
% % by linked prototypes, where the similarities are over a certain
% % threshold δ. Some approaches that do not require a predefined
% % number of classes can also work, such as Louvain [Blondel et
% % al., 2008] and affinity propagation [Frey and Dueck, 2007].
% % To ensure the novel classes are clustered into the same hierarchical level as the known classes, the threshold δ (or the
% % parameter to control the clustering hierarchy) is adjusted automatically by achieving the highest accuracy on the labeled
% % known class samples. With the increasing representation ability of the feature extractor and prototypes, more reliable prototype groups can be obtained gradually.


